Bethe/Gauge Correspondence for ABCDEFG-type 3d Gauge Theories

In this paper, we give a new effective superpotential that makes clear Bethe/Gauge correspondence between 2d (and 3d) $\text{SO/Sp}$ gauge theories and open $\text{XXX}$ (and $\text{XXZ}$) spin chains with diagonal boundary conditions, and also works in the case of 2d (and 3d) $\text{BC}_{N}$-type gauge theories which is not previously discussed in the literature. Especially, for exceptional Lie algebras $\text{F}_{4}$, $\text{G}_{2}$, we give the effective superpotential and vacuum equations. For $\text{E}_{6,7,8}$, we only give theirs effective superpotential for convenience.

==> ref.tex <==
%% This BibTeX bibliography file was created using BibDesk.
%% https://bibdesk.sourceforge.io/

%% Created for zhangting at 2023-03-15 14:54:48 +0800 


%% Saved with string encoding Unicode (UTF-8) 



@article{Fad96,
	archiveprefix = {arXiv},
	author = {Faddeev, L. D.},
	booktitle = {{Les Houches School of Physics: Astrophysical Sources of Gravitational Radiation}},
	date-added = {2023-03-15 14:53:03 +0800},
	date-modified = {2023-03-15 14:54:45 +0800},
	eprint = {hep-th/9605187},
	month = {5},
	pages = {pp. 149--219},
	title = {{How algebraic Bethe ansatz works for integrable model}},
	year = {1996}}

@article{GKMMM95,
	abstract = {The exact Seiberg-Witten (SW) description of the light sector in the N = 2 SUSY 4d Yang-Mills theory [N. Seiberg and E. Witten, Nucl. Phys. B 430 (1994) 485 (E); B 446 (1994) 19] is reformulated in terms of integrable systems and appears to be a Gurevich-Pitaevsky (GP) [A. Gurevich and L. Pitaevsky, JETP 65 (1973) 65; see also, S. Novikov, S. Manakov, L. Pitaevsky and V. Zakharov, Theory of solitons] solution to the elliptic Whitham equations. We consider this as an implication that the dynamical mechanism behind the SW solution is related to integrable systems on the moduli space of instantons. We emphasize the role of the Whitham theory as a possible substitute of the renormalization-group approach to the construction of low-energy effective actions.},
	author = {A. Gorsky and I. Krichever and A. Marshakov and A. Mironov and A. Morozov},
	date-added = {2023-03-15 14:15:28 +0800},
	date-modified = {2023-03-15 14:15:51 +0800},
	doi = {https://doi.org/10.1016/0370-2693(95)00723-X},
	issn = {0370-2693},
	journal = {Physics Letters B},
	number = {3},
	pages = {466-474},
	title = {Integrability and Seiberg-Witten exact solution},
	url = {https://www.sciencedirect.com/science/article/pii/037026939500723X},
	volume = {355},
	year = {1995},
	bdsk-url-1 = {https://www.sciencedirect.com/science/article/pii/037026939500723X},
	bdsk-url-2 = {https://doi.org/10.1016/0370-2693(95)00723-X}}

@article{DZ23,
	author = {Xiang-Mao Ding and Tinglyer Zhang},
	date-added = {2023-03-14 15:29:03 +0800},
	date-modified = {2023-03-14 15:30:30 +0800},
	journal = {arXiv:2303.04575},
	title = {Bethe/Gauge Correspondence for ABCD quiver Gauge Theories and Spin Chains},
	year = {2023}}

@article{YZ06,
	abstract = {We propose that the Baxter's Q-operator for the quantum XYZ spin chain with open boundary conditions is given by the j→∞ limit of the corresponding transfer matrix with spin-j (i.e., (2j+1)-dimensional) auxiliary space. The associated T--Q relation is derived from the fusion hierarchy of the model. We use this relation to determine the Bethe Ansatz solution of the eigenvalues of the fundamental transfer matrix. The solution yields the complete spectrum of the Hamiltonian.},
	author = {Wen-Li Yang and Yao-Zhong ZHang},
	date-added = {2023-03-06 15:12:36 +0800},
	date-modified = {2023-03-06 15:14:07 +0800},
	doi = {https://doi.org/10.1016/j.nuclphysb.2006.03.025},
	issn = {0550-3213},
	journal = {Nuclear Physics B},
	keywords = {Spin chain, Reflection equation, Bethe Ansatz, -operator, Fusion hierarchy},
	number = {3},
	pages = {312-329},
	title = {T--Q relation and exact solution for the XYZ chain with general non-diagonal boundary terms},
	url = {https://www.sciencedirect.com/science/article/pii/S0550321306002380},
	volume = {744},
	year = {2006},
	bdsk-url-1 = {https://www.sciencedirect.com/science/article/pii/S0550321306002380},
	bdsk-url-2 = {https://doi.org/10.1016/j.nuclphysb.2006.03.025}}

@article{OR11,
	abstract = {The Gauge/Bethe correspondence of Nekrasov and Shatashvili relates the spectrum of integrable spin chains to the ground states of supersymmetric gauge theories. Up to now, this correspondence has been an observation; the underlying reason for its existence remaining elusive. We argue here that geometrical representation theory is a mathematical foundation of the Gauge/Bethe correspondence, and it provides a framework to study families of gauge theories in a unified way.},
	author = {Orlando, Domenico and Reffert, Susanne},
	date = {2011/12/01},
	date-added = {2023-02-27 19:36:11 +0800},
	date-modified = {2023-02-27 19:36:27 +0800},
	doi = {10.1007/s11005-011-0526-5},
	id = {Orlando2011},
	isbn = {1573-0530},
	journal = {Letters in Mathematical Physics},
	number = {3},
	pages = {289--298},
	title = {The Gauge--Bethe Correspondence and Geometric Representation Theory},
	url = {https://doi.org/10.1007/s11005-011-0526-5},
	volume = {98},
	year = {2011},
	bdsk-url-1 = {https://doi.org/10.1007/s11005-011-0526-5}}

@article{Mac03,
	author = {L.G.Macdonald},
	date-added = {2023-02-27 18:37:11 +0800},
	date-modified = {2023-02-27 18:39:07 +0800},
	journal = {Cambridge University Press},
	number = {157},
	title = {Affine Hecke algebras and orthogonal polynomials},
	year = {2003}}

@article{Hum72,
	author = {J.Humphreys},
	date-added = {2023-02-22 19:21:28 +0800},
	date-modified = {2023-02-22 19:22:26 +0800},
	title = {Introduction to Lie Algebra and Representation Theory},
	year = {1972}}

@article{WYC15,
	author = {Y. Wang, W. L. Yang, J. Cao et al},
	date-added = {2023-02-02 18:01:42 +0800},
	date-modified = {2023-02-02 18:04:04 +0800},
	title = {Off-diagonal Bethe Ansatz for exactly solvable models},
	year = {2015}}

@article{YS20,
	author = {Yutaka Yoshida and Katsuyuki Sugiyama},
	date-added = {2023-02-02 18:01:32 +0800},
	date-modified = {2023-02-02 18:07:23 +0800},
	journal = {Progress of Theoretical and Experimental Physics},
	number = {11},
	title = {Localization of three-dimensional N=2 supersymmetry theories on S1*D2},
	volume = {2020},
	year = {2020}}

@article{Wit89,
	author = {E. Witten},
	date-added = {2023-02-02 17:59:51 +0800},
	date-modified = {2023-02-02 18:00:35 +0800},
	journal = {Nuclear Physics B},
	number = {3},
	pages = {629--697},
	title = {Gauge theories and integrable lattice models},
	volume = {322},
	year = {1989}}

@article{SW94b,
	abstract = {We study four dimensional N = 2 supersymmetric gauge theories with matter multiplets. For all such models for which the gauge group is SU(2), we derive the exact metric on the moduli space of quantum vacua and the exact spectrum of the stable massive states. A number of new physical phenomena occur, such as chiral symmetry breaking that is driven by the condensation of magnetic monopoles that carry global quantum numbers. For those cases in which conformal invariance is broken only by mass terms, the formalism automatically gives results that are invariant under electric-magnetic duality. In one instance, this duality is mixed in an interesting way with SO(8) triality.},
	author = {N. Seiberg and E. Witten},
	date-added = {2023-02-02 17:59:00 +0800},
	date-modified = {2023-02-02 17:59:12 +0800},
	doi = {https://doi.org/10.1016/0550-3213(94)90214-3},
	issn = {0550-3213},
	journal = {Nuclear Physics B},
	number = {3},
	pages = {484-550},
	title = {Monopoles, duality and chiral symmetry breaking in N = 2 supersymmetric QCD},
	url = {https://www.sciencedirect.com/science/article/pii/0550321394902143},
	volume = {431},
	year = {1994},
	bdsk-url-1 = {https://www.sciencedirect.com/science/article/pii/0550321394902143},
	bdsk-url-2 = {https://doi.org/10.1016/0550-3213(94)90214-3}}

@article{SW94a,
	abstract = {We study the vacuum structure and don spectrum of N=2 supersymmetric gauge theory in four dimensions, with gauge group SU(2). The theory turns out to have remarkably rich and physical properties which can nonetheless be described precisely; exact formulas can be obtained, for instance, for electron and dyon masses and the metric on the moduli space of vacua. The description involves a version of Olive-Montonen electric-magnetic duality. The ``strongly coupled'' vacuum turns out to be a weakly coupled theory of monopoles, and with a suitable perturbation confinement is described by monopole condensation.},
	author = {N. Seiberg and E. Witten},
	date-added = {2023-02-02 17:57:33 +0800},
	date-modified = {2023-02-02 17:57:53 +0800},
	doi = {https://doi.org/10.1016/0550-3213(94)90124-4},
	issn = {0550-3213},
	journal = {Nuclear Physics B},
	number = {1},
	pages = {19-52},
	title = {Electric-magnetic duality, monopole condensation, and confinement in N=2 supersymmetric Yang-Mills theory},
	url = {https://www.sciencedirect.com/science/article/pii/0550321394901244},
	volume = {426},
	year = {1994},
	bdsk-url-1 = {https://www.sciencedirect.com/science/article/pii/0550321394901244},
	bdsk-url-2 = {https://doi.org/10.1016/0550-3213(94)90124-4}}

@article{Sun18,
	abstract = {By combining the algebraic Bethe ansatz and the off-diagonal Bethe ansatz, we investigate the trigonometric SU(3) model with generic open boundaries. The eigenvalues of the transfer matrix are given in terms of an inhomogeneous T−Q relation, and the corresponding eigenstates are expressed in terms of nested Bethe-type eigenstates which have well-defined homogeneous limit. This exact solution provides a basis for further analyzing the thermodynamic properties and correlation functions of the anisotropic models associated with higher rank algebras.},
	author = {Pei Sun and Zhirong Xin and Yi Qiao and Fakai Wen and Kun Hao and Junpeng Cao and Guang-Liang Li and Tao Yang and Wen-Li Yang and Kangjie Shi},
	date-added = {2023-02-02 17:56:31 +0800},
	date-modified = {2023-02-02 17:56:40 +0800},
	doi = {https://doi.org/10.1016/j.nuclphysb.2018.04.025},
	issn = {0550-3213},
	journal = {Nuclear Physics B},
	pages = {342-358},
	title = {Bethe states of the trigonometric SU(3) spin chain with generic open boundaries},
	url = {https://www.sciencedirect.com/science/article/pii/S0550321318301263},
	volume = {931},
	year = {2018},
	bdsk-url-1 = {https://www.sciencedirect.com/science/article/pii/S0550321318301263},
	bdsk-url-2 = {https://doi.org/10.1016/j.nuclphysb.2018.04.025}}

@article{Skl88,
	author = {E.K. Sklyanin},
	date-added = {2023-02-02 17:54:44 +0800},
	date-modified = {2023-02-02 17:55:39 +0800},
	journal = {Journal of Physics A: Mathematical and General},
	number = {10},
	pages = {2375},
	title = {Boundary Conditions for Integrable Quantum Systems},
	volume = {21},
	year = {1988}}

@article{NW10,
	abstract = {We reformulate the Ω-deformation of four-dimensional gauge theory in a way that is valid away from fixed points of the associated group action. We use this reformulation together with the theory of coisotropic A-branes to explain recent results linking the Ω-deformation to integrable Hamiltonian systems in one direction and Liouville theory of two-dimensional conformal field theory in another direction.},
	author = {Nekrasov, Nikita and Witten, Edward},
	date = {2010/09/27},
	date-added = {2023-02-02 17:53:22 +0800},
	date-modified = {2023-02-02 17:53:27 +0800},
	doi = {10.1007/JHEP09(2010)092},
	id = {Nekrasov2010},
	isbn = {1029-8479},
	journal = {Journal of High Energy Physics},
	number = {9},
	pages = {92},
	title = {The omega deformation, branes, integrability and Liouville theory},
	url = {https://doi.org/10.1007/JHEP09(2010)092},
	volume = {2010},
	year = {2010},
	bdsk-url-1 = {https://doi.org/10.1007/JHEP09(2010)092}}

@article{NVS18,
	abstract = {We study macroscopically two dimensional {\$}{\$}{\{}{$\backslash$}mathcal{\{}N{\}}=(2,2){\}}{\$}{\$}supersymmetric gauge theories constructed by compactifying the quiver gauge theories with eight supercharges on a product {\$}{\$}{\{}{$\backslash$}mathbb{\{}T{\}}\^{}{\{}d{\}} {$\backslash$}times {$\backslash$}mathbb{\{}R{\}}\^{}{\{}2{\}}{\_}{\{}{$\backslash$}epsilon{\}}{\}}{\$}{\$}of a d-dimensional torus and a two dimensional cigar with {\$}{\$}{\{}{$\backslash$}Omega{\}}{\$}{\$}-deformation. We compute the universal part of the effective twisted superpotential. In doing so we establish the correspondence between the gauge theories and the Yangian {\$}{\$}{\{}{$\backslash$}mathbf{\{}Y{\}}{\_}{\{}{$\backslash$}epsilon{\}}({$\backslash$}mathfrak{\{}g{\}}{\_}{\{}{$\backslash$}Gamma{\}}){\}}{\$}{\$}, quantum affine algebra {\$}{\$}{\{}{$\backslash$}mathbf{\{}U{\}}\^{}{\{}{$\backslash$}mathrm{\{}aff{\}}{\}}{\_}q({$\backslash$}mathfrak{\{}g{\}}{\_}{\{}{$\backslash$}Gamma{\}}){\}}{\$}{\$}, or the quantum elliptic algebra {\$}{\$}{\{}{$\backslash$}mathbf{\{}U{\}}\^{}{\{}{$\backslash$}mathrm{\{}ell{\}}{\}}{\_}{\{}q,p{\}}({$\backslash$}mathfrak{\{}g{\}}{\_}{\{}{$\backslash$}Gamma{\}}){\}}{\$}{\$}associated to Kac--Moody algebra {\$}{\$}{\{}{$\backslash$}mathfrak{\{}g{\}}{\_}{\{}{$\backslash$}Gamma{\}}{\}}{\$}{\$}for quiver {\$}{\$}{\{}{$\backslash$}Gamma{\}}{\$}{\$}.},
	author = {Nekrasov, Nikita and Pestun, Vasily and Shatashvili, Samson},
	date = {2018/01/01},
	date-added = {2023-02-02 17:52:19 +0800},
	date-modified = {2023-02-02 17:52:40 +0800},
	doi = {10.1007/s00220-017-3071-y},
	id = {Nekrasov2018},
	isbn = {1432-0916},
	journal = {Communications in Mathematical Physics},
	number = {2},
	pages = {519--567},
	title = {Quantum Geometry and Quiver Gauge Theories},
	url = {https://doi.org/10.1007/s00220-017-3071-y},
	volume = {357},
	year = {2018},
	bdsk-url-1 = {https://doi.org/10.1007/s00220-017-3071-y}}

@article{NS09c,
	abstract = { Abstract We study four dimensional \$\mathcal{N} = 2\$ supersymmetric gauge theory in the Ω-background with the two dimensional \$\mathcal{N} = 2\$ super-Poincare invariance. We explain how this gauge theory provides the quantization of the classical integrable system underlying the moduli space of vacua of the ordinary four dimensional \$\mathcal{N} = 2\$ theory. The ε-parameter is identified with the Planck constant, the twisted chiral ring maps to quantum Hamiltonians, the supersymmetric vacua are identified with Bethe states of quantum integrable systems. This four dimensional gauge theory in its low energy description has two dimensional twisted superpotential on Σ which becomes the Yang-Yang function of the integrable system. We present the thermodynamic-Bethe-Ansatz like formulae for these functions and the spectra of commuting Hamiltonians following the direct computation in gauge theory. The general construction is illustrated at the examples of the many-body systems, such as the periodic Toda chain, the elliptic Calogero-Moser system, and their relativistic versions, for which we present a complete characterization of the L2-spectrum. We very briefly discuss the quantization of Hitchin system. },
	author = {NIKITA A. NEKRASOV and SAMSON L. SHATASHVILI},
	booktitle = {XVIth International Congress on Mathematical Physics},
	date-added = {2023-02-02 17:50:53 +0800},
	date-modified = {2023-02-02 17:51:02 +0800},
	doi = {10.1142/9789814304634_0015},
	eprint = {https://www.worldscientific.com/doi/pdf/10.1142/9789814304634_0015},
	pages = {265-289},
	title = {QUANTIZATION OF INTEGRABLE SYSTEMS AND FOUR DIMENSIONAL GAUGE THEORIES},
	url = {https://www.worldscientific.com/doi/abs/10.1142/9789814304634_0015},
	bdsk-url-1 = {https://www.worldscientific.com/doi/abs/10.1142/9789814304634_0015},
	bdsk-url-2 = {https://doi.org/10.1142/9789814304634_0015}}

@article{NS09b,
	author = {N. Nekrasov and Samson L.Shatashvili},
	date-added = {2023-02-02 17:47:19 +0800},
	date-modified = {2023-02-02 17:49:21 +0800},
	journal = {AIP Conference Proceedings},
	pages = {154--169},
	title = {Bethe Ansatz and supersymmetric vacua},
	volume = {1134},
	year = {2009}}

@article{NS09a,
	author = {N. Nekrasov and Samson L.Shatashvili},
	date-added = {2023-02-02 17:44:37 +0800},
	date-modified = {2023-02-02 17:46:06 +0800},
	journal = {Nuclear Physics B},
	pages = {91--112},
	title = {Supersymmetric vacua and Bethe ansatz},
	volume = {192-193},
	year = {2009}}

@article{NRS11,
	abstract = {The moduli space of SL2 flat connections on a punctured Riemann surface Σ with the fixed conjugacy classes of the monodromies around the punctures is endowed with a system of holomorphic Darboux coordinates, in which the generating function of the variety of SL2-opers is identified with the universal part of the effective twisted superpotential of the Gaiotto type four dimensional N=2 supersymmetric theory subject to the two-dimensional Ω-deformation. This allows to give a definition of the Yang-Yang functionals for the quantum Hitchin system in terms of the classical geometry of the moduli space of local systems for the dual gauge group, and connect it to the instanton counting of the four dimensional gauge theories, in the rank one case.},
	author = {N. Nekrasov and A. Rosly and S. Shatashvili},
	date-added = {2023-02-02 17:43:39 +0800},
	date-modified = {2023-02-02 17:43:50 +0800},
	doi = {https://doi.org/10.1016/j.nuclphysbps.2011.04.150},
	issn = {0920-5632},
	journal = {Nuclear Physics B - Proceedings Supplements},
	note = {String Theory: Formal Developments and Applications},
	number = {1},
	pages = {69-93},
	title = {Darboux coordinates, Yang-Yang functional, and gauge theory},
	url = {https://www.sciencedirect.com/science/article/pii/S0920563211004269},
	volume = {216},
	year = {2011},
	bdsk-url-1 = {https://www.sciencedirect.com/science/article/pii/S0920563211004269},
	bdsk-url-2 = {https://doi.org/10.1016/j.nuclphysbps.2011.04.150}}

@article{NPS18,
	abstract = {We study macroscopically two dimensional {\$}{\$}{\{}{$\backslash$}mathcal{\{}N{\}}=(2,2){\}}{\$}{\$}supersymmetric gauge theories constructed by compactifying the quiver gauge theories with eight supercharges on a product {\$}{\$}{\{}{$\backslash$}mathbb{\{}T{\}}\^{}{\{}d{\}} {$\backslash$}times {$\backslash$}mathbb{\{}R{\}}\^{}{\{}2{\}}{\_}{\{}{$\backslash$}epsilon{\}}{\}}{\$}{\$}of a d-dimensional torus and a two dimensional cigar with {\$}{\$}{\{}{$\backslash$}Omega{\}}{\$}{\$}-deformation. We compute the universal part of the effective twisted superpotential. In doing so we establish the correspondence between the gauge theories and the Yangian {\$}{\$}{\{}{$\backslash$}mathbf{\{}Y{\}}{\_}{\{}{$\backslash$}epsilon{\}}({$\backslash$}mathfrak{\{}g{\}}{\_}{\{}{$\backslash$}Gamma{\}}){\}}{\$}{\$}, quantum affine algebra {\$}{\$}{\{}{$\backslash$}mathbf{\{}U{\}}\^{}{\{}{$\backslash$}mathrm{\{}aff{\}}{\}}{\_}q({$\backslash$}mathfrak{\{}g{\}}{\_}{\{}{$\backslash$}Gamma{\}}){\}}{\$}{\$}, or the quantum elliptic algebra {\$}{\$}{\{}{$\backslash$}mathbf{\{}U{\}}\^{}{\{}{$\backslash$}mathrm{\{}ell{\}}{\}}{\_}{\{}q,p{\}}({$\backslash$}mathfrak{\{}g{\}}{\_}{\{}{$\backslash$}Gamma{\}}){\}}{\$}{\$}associated to Kac--Moody algebra {\$}{\$}{\{}{$\backslash$}mathfrak{\{}g{\}}{\_}{\{}{$\backslash$}Gamma{\}}{\}}{\$}{\$}for quiver {\$}{\$}{\{}{$\backslash$}Gamma{\}}{\$}{\$}.},
	author = {Nekrasov, Nikita and Pestun, Vasily and Shatashvili, Samson},
	date = {2018/01/01},
	date-added = {2023-02-02 17:40:31 +0800},
	date-modified = {2023-02-02 17:40:44 +0800},
	doi = {10.1007/s00220-017-3071-y},
	id = {Nekrasov2018},
	isbn = {1432-0916},
	journal = {Communications in Mathematical Physics},
	number = {2},
	pages = {519--567},
	title = {Quantum Geometry and Quiver Gauge Theories},
	url = {https://doi.org/10.1007/s00220-017-3071-y},
	volume = {357},
	year = {2018},
	bdsk-url-1 = {https://doi.org/10.1007/s00220-017-3071-y}}

@article{NP12,
	author = {N. Nekrasov and Vasily Pestun},
	date-added = {2023-02-02 17:36:54 +0800},
	date-modified = {2023-02-02 17:38:27 +0800},
	journal = {arxiv:1211.1240},
	title = {Seiberg-Witten geometry of four dimensional N=2 quiver gauge theories},
	year = {2012}}

@article{NN21,
	abstract = {The relation between supersymmetric gauge theories in four dimensions and quantum spin systems is exploited to find an explicit formula for the Jost function of the N site {\$}{\$} {$\backslash$}mathfrak{\{}sl{\}} {\$}{\$}2 X X X spin chain (for infinite dimensional complex spin representations), as well as the SLN Gaudin system, which reduces, in a limiting case, to that of the N-particle periodic Toda chain. Using the non-perturbative Dyson-Schwinger equations of the supersymmetric gauge theory we establish relations between the spin chain commuting Hamiltonians with the twisted chiral ring of gauge theory. Along the way we explore the chamber dependence of the supersymmetric partition function, also the expectation value of the surface defects, giving new evidence for the AGT conjecture.},
	author = {Lee, Norton and Nekrasov, Nikita},
	date = {2021/03/09},
	date-added = {2023-02-02 17:34:38 +0800},
	date-modified = {2023-02-02 17:34:48 +0800},
	doi = {10.1007/JHEP03(2021)093},
	id = {Lee2021},
	isbn = {1029-8479},
	journal = {Journal of High Energy Physics},
	number = {3},
	pages = {93},
	title = {Quantum spin systems and supersymmetric gauge theories. Part I},
	url = {https://doi.org/10.1007/JHEP03(2021)093},
	volume = {2021},
	year = {2021},
	bdsk-url-1 = {https://doi.org/10.1007/JHEP03(2021)093}}

@article{Nek19,
	abstract = {Quantum field theory {\$}{\$}L{\_}1{\$}{\$}on spacetime {\$}{\$}X{\_}{\{}1{\}}{\$}{\$}can be coupled to another quantum field theory {\$}{\$}L{\_}2{\$}{\$}on a spacetime {\$}{\$}X{\_}{\{}2{\}}{\$}{\$}via the third quantum field theory {\$}{\$}L{\_}{\{}12{\}}{\$}{\$}living on {\$}{\$}X{\_}{\{}12{\}} = X{\_}{\{}1{\}} {$\backslash$}cap X{\_}{\{}2{\}}{\$}{\$}. We explore several such constructions with two- and four-dimensional {\$}{\$}X{\_}{\{}1{\}}, X{\_}{\{}2{\}}{\$}{\$}'s and zero- and two-dimensional {\$}{\$}X{\_}{\{}12{\}}{\$}{\$}'s, in the context of {\$}{\$}{\{}{$\backslash$}mathcal {\{}N{\}}{\}}=2{\$}{\$}supersymmetry, non-perturbative Dyson--Schwinger equations, and BPS/CFT correspondence. The companion paper (Nekrasov, ``BPS/CFT correspondence V: BPZ and KZ equations from qq-characters'', 2017. arXiv:1711.11582{$[$}hep-th{$]$}) will show that the BPZ and KZ equations of two-dimensional conformal field theory are obeyed by the half-BPS surface defects in quiver {\$}{\$}{\{}{$\backslash$}mathcal {\{}N{\}}{\}}=2{\$}{\$}gauge theories.},
	author = {Nekrasov, Nikita},
	date = {2019/03/01},
	date-added = {2023-02-02 17:33:27 +0800},
	date-modified = {2023-02-02 17:33:35 +0800},
	doi = {10.1007/s11005-018-1115-7},
	id = {Nekrasov2019},
	isbn = {1573-0530},
	journal = {Letters in Mathematical Physics},
	number = {3},
	pages = {579--622},
	title = {BPS/CFT correspondence IV: sigma models and defects in gauge theory},
	url = {https://doi.org/10.1007/s11005-018-1115-7},
	volume = {109},
	year = {2019},
	bdsk-url-1 = {https://doi.org/10.1007/s11005-018-1115-7}}

@article{Nek18,
	abstract = {We study generalized gauge theories engineered by taking the low energy limit of the Dp branes wrapping {\$}{\$}{\{}X {$\backslash$}times {\{}{$\backslash$}bf T{\}}\^{}{\{}p-3{\}}{\}}{\$}{\$}, with X a possibly singular surface in a Calabi--Yau fourfold Z. For toric Z and X the partition function can be computed by localization, making it a statistical mechanical model, called the {\$}{\$}{\{}{$\backslash$}underline{\{}{$\backslash$}rm gauge{$\backslash$},origami{\}}{\}}{\$}{\$}. The random variables are the ensembles of Young diagrams. The building block of the gauge origami is associated with a tetrahedron, whose edges are colored by vector spaces. We show the properly normalized partition function is an entire function of the Coulomb moduli, for generic values of the {\$}{\$}{\{}{$\backslash$}Omega{\}}{\$}{\$}-background parameters. The orbifold version of the theory defines the qq-character operators, with and without the surface defects. The analytic properties are the consequence of a relative compactness of the moduli spaces {\$}{\$}{\{}{$\backslash$}mathcal{\{}M{\}}({\{}{$\backslash$}vec n{\}}, k){\}}{\$}{\$}of crossed and spiked instantons, demonstrated in ``BPS/CFT correspondence II: instantons at crossroads, moduli and compactness theorem''.},
	author = {Nekrasov, Nikita},
	date = {2018/03/01},
	date-added = {2023-02-02 17:32:47 +0800},
	date-modified = {2023-02-02 17:32:54 +0800},
	doi = {10.1007/s00220-017-3057-9},
	id = {Nekrasov2018},
	isbn = {1432-0916},
	journal = {Communications in Mathematical Physics},
	number = {3},
	pages = {863--894},
	title = {BPS/CFT Correspondence III: Gauge Origami Partition Function and qq-Characters},
	url = {https://doi.org/10.1007/s00220-017-3057-9},
	volume = {358},
	year = {2018},
	bdsk-url-1 = {https://doi.org/10.1007/s00220-017-3057-9}}

@article{Nek17b,
	author = {N. Nekrasov},
	date-added = {2023-02-02 17:31:27 +0800},
	date-modified = {2023-02-02 17:32:10 +0800},
	journal = {arXiv:1711.11582},
	title = {{BPS/CFT correspondence V: BPZ and KZ equations from qq-characters}},
	year = {2017}}

@article{Nek17a,
	author = {N. Nekrasov},
	date-added = {2023-02-02 17:28:46 +0800},
	date-modified = {2023-02-02 17:30:37 +0800},
	journal = {arXiv:1608.07272},
	title = {{BPS/CFT CORRESPONDENCE II: INSTANTONS AT CROSSROADS, MODULI AND COMPACTNESS THEOREM}},
	year = {2017}}

@article{Nek16,
	abstract = {We study symmetries of quantum field theories involving topologically distinct sectors of the field space. To exhibit these symmetries we define special gauge invariant observables, which we call the qq-characters. In the context of the BPS/CFT correspondence, using these observables, we derive an infinite set of Dyson-Schwinger-type relations. These relations imply that the supersymmetric partition functions in the presence of Ω-deformation and defects obey the Ward identities of two dimensional conformal field theory and its q-deformations. The details will be discussed in the companion papers.},
	author = {Nekrasov, Nikita},
	date = {2016/03/25},
	date-added = {2023-02-02 17:27:57 +0800},
	date-modified = {2023-02-02 17:28:04 +0800},
	doi = {10.1007/JHEP03(2016)181},
	id = {Nekrasov2016},
	isbn = {1029-8479},
	journal = {Journal of High Energy Physics},
	number = {3},
	pages = {181},
	title = {BPS/CFT correspondence: non-perturbative Dyson-Schwinger equations and qq-characters},
	url = {https://doi.org/10.1007/JHEP03(2016)181},
	volume = {2016},
	year = {2016},
	bdsk-url-1 = {https://doi.org/10.1007/JHEP03(2016)181}}

@article{Nek04,
	author = {N. Nekrasov},
	date-added = {2023-02-02 17:24:42 +0800},
	date-modified = {2023-02-02 17:27:03 +0800},
	journal = {arXiv hep-th/0306211},
	title = {Seiberg-Witten prepotential from instanton counting},
	year = {2003}}

@article{MNS00,
	abstract = {We develop some useful techniques for integrating over Higgs branches in supersymmetric theories with 4 and 8 supercharges. In particular, we define a regularized volume for hyperk{\"a}hler quotients. We evaluate this volume for certain ALE and ALF spaces in terms of the hyperk{\"a}hler periods. We also reduce these volumes for a large class of hyperk{\"a}hler quotients to  simpler integrals. These quotients include complex coadjoint orbits, instanton  moduli spaces on ℝ4 and ALE manifolds, Hitchin spaces, and moduli spaces of (parabolic) Higgs bundles on Riemann surfaces. In the case of Hitchin spaces the evaluation of the volume reduces to a summation over solutions of Bethe Ansatz equations for the non-linear Schr{\"o}dinger system. We discuss some applications of our results.},
	author = {Moore, Gregory and Nekrasov, Nikita and Shatashvili, Samson},
	date = {2000/01/01},
	date-added = {2023-02-02 17:23:20 +0800},
	date-modified = {2023-02-02 17:23:35 +0800},
	doi = {10.1007/PL00005525},
	id = {Moore2000},
	isbn = {1432-0916},
	journal = {Communications in Mathematical Physics},
	number = {1},
	pages = {97--121},
	title = {Integrating over Higgs Branches},
	url = {https://doi.org/10.1007/PL00005525},
	volume = {209},
	year = {2000},
	bdsk-url-1 = {https://doi.org/10.1007/PL00005525}}

@article{LNP19,
	abstract = {We consider 4d {\$}{\$} {$\backslash$}mathcal{\{}N{\}} {\$}{\$}= 1 gauge theories with R-symmetry on a hemisphere times a torus. We apply localization techniques to evaluate the exact partition function through a cohomological reformulation of the supersymmetry transformations. Our results represent the natural elliptic lifts of the lower dimensional analogs as well as a field theoretic derivation of the conjectured 4d holomorphic blocks, from which partition functions of compact spaces with diverse topology can be recovered through gluing. We also analyze the different boundary conditions which can naturally be imposed on the chiral multiplets, which turn out to be either Dirichlet or Robin-like. We show that different boundary conditions are related to each other by coupling the bulk to 3d {\$}{\$} {$\backslash$}mathcal{\{}N{\}} {\$}{\$}= 1 degrees of freedom on the boundary three-torus, for which we derive explicit 1-loop determinants.},
	author = {Longhi, Pietro and Nieri, Fabrizio and Pittelli, Antonio},
	date = {2019/12/20},
	date-added = {2023-02-02 17:20:08 +0800},
	date-modified = {2023-02-02 17:20:34 +0800},
	doi = {10.1007/JHEP12(2019)147},
	id = {Longhi2019},
	isbn = {1029-8479},
	journal = {Journal of High Energy Physics},
	number = {12},
	pages = {147},
	title = {Localization of 4d {\$}{\$} {$\backslash$}mathcal{\{}N{\}} {\$}{\$}= 1 theories on 𝔻2×𝕋2},
	url = {https://doi.org/10.1007/JHEP12(2019)147},
	volume = {2019},
	year = {2019},
	bdsk-url-1 = {https://doi.org/10.1007/JHEP12(2019)147}}

@article{KZ21,
	abstract = {In this article, we extend the work of {$[$}1{$]$} to a Bethe/Gauge correspondence between 2d (or resp. 3d) SO/Sp gauge theories and open XXX (resp. XXZ) spin chains with diagonal boundary conditions. The case of linear quiver gauge theories is also considered.},
	author = {Kimura, Taro and Zhu, Rui-Dong},
	date = {2021/03/24},
	date-added = {2023-02-02 17:18:52 +0800},
	date-modified = {2023-02-02 17:18:58 +0800},
	doi = {10.1007/JHEP03(2021)227},
	id = {Kimura2021},
	isbn = {1029-8479},
	journal = {Journal of High Energy Physics},
	number = {3},
	pages = {227},
	title = {Bethe/gauge correspondence for SO/Sp gauge theories and open spin chains},
	url = {https://doi.org/10.1007/JHEP03(2021)227},
	volume = {2021},
	year = {2021},
	bdsk-url-1 = {https://doi.org/10.1007/JHEP03(2021)227}}

@article{IK94,
	author = {Inami, Takeo and Konno, Hitoshi},
	date-added = {2023-02-02 17:10:22 +0800},
	date-modified = {2023-02-08 16:21:43 +0800},
	journal = {Journal of Physics A: Mathematical and General},
	number = {24},
	title = {Integrable XYZ spin chain with boundaries},
	volume = {27},
	year = {1994}}

@article{GS08b,
	author = {Gerasimov, Anton A and Shatashvili, Samson L},
	date-added = {2023-02-02 17:05:38 +0800},
	date-modified = {2023-02-02 17:08:07 +0800},
	journal = {arXiv preprint arXiv:0711.1472},
	title = {Two-dimensional Gauge Theories and Quantum Integrable Systems},
	year = {2007}}

@article{GS08a,
	abstract = {The appearance of the Bethe Ansatz equation for the Nonlinear Schr{\"o}dinger equation in the equivariant integration over the moduli space of Higgs bundles is revisited. We argue that the wave functions of the corresponding two-dimensional topological U(N) gauge theory reproduce quantum wave functions of the Nonlinear Schr{\"o}dinger equation in the N-particle sector. This implies the full equivalence between the above gauge theory and the N-particle sub-sector of the quantum theory of the Nonlinear Schr{\"o}dinger equation. This also implies the explicit correspondence between the gauge theory and the representation theory of the degenerate double affine Hecke algebra. We propose a similar construction based on the G/G gauged WZW model leading to the representation theory of the double affine Hecke algebra.},
	author = {Gerasimov, Anton A. and Shatashvili, Samson L.},
	date = {2008/01/01},
	date-added = {2023-02-02 17:04:43 +0800},
	date-modified = {2023-02-02 17:05:32 +0800},
	doi = {10.1007/s00220-007-0369-1},
	id = {Gerasimov2008},
	isbn = {1432-0916},
	journal = {Communications in Mathematical Physics},
	number = {2},
	pages = {323--367},
	title = {Higgs Bundles, Gauge Theories and Quantum Groups},
	url = {https://doi.org/10.1007/s00220-007-0369-1},
	volume = {277},
	year = {2008},
	bdsk-url-1 = {https://doi.org/10.1007/s00220-007-0369-1}}

@article{GN95,
	author = {A. Gorsky and A. Nekrasov},
	date-added = {2023-02-02 17:02:41 +0800},
	date-modified = {2023-02-02 17:03:35 +0800},
	journal = {Nuclear Physics B},
	number = {3},
	pages = {582--608},
	title = {Relativistic Calogero--Moser model as gauged WZW theory},
	volume = {436},
	year = {1995}}

@article{GN94b,
	author = {A. Gorsky and A. Nekrasov},
	date-added = {2023-02-02 17:00:50 +0800},
	date-modified = {2023-02-02 17:02:08 +0800},
	journal = {arXiv preprint hep-th/9401021},
	title = {Elliptic Calogero--Moser system from two-dimensional current algebra},
	year = {1994}}

@article{GN94a,
	author = {A. Gorsky and N. Nekrasov},
	date-added = {2023-02-02 16:58:08 +0800},
	date-modified = {2023-02-02 16:59:52 +0800},
	journal = {Nuclear Physics B},
	number = {1-2},
	pages = {213--238},
	title = {Hamiltonian systems of Calogero type and two-dimensional Yang--Mills theory},
	volume = {414},
	year = {1994}}

@article{FHSY96,
	author = {Fan, Heng and Hou, Bo-yu and Shi, Kang-jie and Yang, Zhong-xia},
	date-added = {2023-02-02 16:52:41 +0800},
	date-modified = {2023-02-02 16:55:01 +0800},
	journal = {Nuclear Physics B},
	number = {3},
	pages = {723--757},
	title = {Algebraic Bethe ansatz for the eight-vertex model with general open boundary conditions},
	volume = {478},
	year = {1996}}

@article{Bax07,
	author = {R. Baxter},
	date-added = {2023-02-02 16:49:35 +0800},
	date-modified = {2023-02-02 16:52:11 +0800},
	title = {Exactly Solved Models in Statistical Mechanics},
	year = {2016}}

